A General Framework for Verification and Control of Dynamical Models via Certificate Synthesis

An emerging branch of control theory specialises in certificate learning, concerning the specification of a desired (possibly complex) system behaviour for an autonomous or control model, which is then analytically verified by means of a function-based proof. However, the synthesis of controllers abiding by these complex requirements is in general a non-trivial task and may elude the most expert control engineers. This results in a need for automatic techniques that are able to design controllers and to analyse a wide range of elaborate specifications. In this paper, we provide a general framework to encode system specifications and define corresponding certificates, and we present an automated approach to formally synthesise controllers and certificates. Our approach contributes to the broad field of safe learning for control, exploiting the flexibility of neural networks to provide candidate control and certificate functions, whilst using SMT-solvers to offer a formal guarantee of correctness. We test our framework by developing a prototype software tool, and assess its efficacy at verification via control and certificate synthesis over a large and varied suite of benchmarks.

==> premable.tex <==
\usepackage[utf8]{inputenc}

\usepackage{generic}
\usepackage[utf8]{inputenc}
\usepackage{amsmath,amssymb,amsfonts}

\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{mathtools}
\usepackage{nccmath}

\usepackage{tikz}
\usetikzlibrary{hobby,decorations.markings}
\usepackage[]{pgfplots}
\pgfplotsset{compat=newest}
\usepackage{pifont}
\usepackage{nicefrac}
\usepackage{tabularx}
\usepackage{multirow}
\usepackage{booktabs}

\usepackage[colorlinks=true]{hyperref}
\renewcommand{\QED}{\square}

\newcommand{\aed}{\textcolor{purple}}
\definecolor{dgreen}{RGB}{61,152,56}

\setlength{\paperheight}{297mm}
\setlength{\paperwidth}{210mm}


\newcommand{\ape}{\textcolor{blue}}
\newcommand{\red}{\textcolor{red}}
\newcommand{\blue}{\textcolor{blue}}
\newcommand{\ale}{\textcolor{red}}


\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}

\newcommand{\cX}{\mathcal{X}}
\newcommand{\cI}{\mathcal{X}_I}
\newcommand{\cB}{\mathcal{X}_B}
\newcommand{\cG}{\mathcal{X}_G}
\newcommand{\cS}{\mathcal{X}_S}
\newcommand{\cU}{\mathcal{X}_U}
\newcommand{\cF}{\mathcal{X}_F}
\newcommand{\real}{\mathbb{R}}
\newcommand{\extreal}{\overline{\mathbb{R}}}
\newcommand{\relu}{\text{ReLU}}



\newtheorem{theorem}{\bfseries Theorem}
\newtheorem{corollary}[theorem]{\bfseries Corollary}%
\newtheorem{remark}[theorem]{\bfseries Remark}
\newtheorem{certificate}{\bfseries Certificate}
\newtheorem{example}{\bfseries Example}%




\usetikzlibrary[patterns.meta, positioning, hobby, calc, arrows.meta, decorations.pathreplacing, backgrounds, matrix, calligraphy, shapes.misc]

